Entropy-Stable and Physical-Constraint-Preserving DGSEM for Symmetry-Reduced General-Relativistic Hydrodynamics on Stationary Spacetimes

We develop an entropy-stable and physical-constraint-preserving discontinuous Galerkin spectral element method for symmetry-reduced general-relativistic hydrodynamics on prescribed stationary spacetimes. Using a local orthonormal transformation, the fluid variables are expressed in a form for which the relativistic hydrodynamic algebra and the admissible set are independent of the spatial metric, while the spacetime geometry enters through stationary coefficients. This separation allows entropy-conservative special-relativistic fluxes to be combined with a compatible discretization of the geometric source terms. On affine tensor-product meshes, the resulting DGSEM is conservative and satisfies a semidiscrete entropy inequality, while the transformed variables provide a convex framework for physical-constraint preservation. For practical stabilization, we use a geometry-only causal speed that is sufficient for both classical local Lax--Friedrichs entropy dissipation and the physical-constraint-preserving Lax--Friedrichs splitting. The fully discrete method combines this stabilization with SSP Runge--Kutta time stepping, oscillation elimination, and conservative local-orthonormal-state scaling. Numerical experiments cover smooth and strongly shocked special-relativistic flows, an axisymmetric jet, stationary Michel accretion, Schwarzschild Bondi--Hoyle flow, and four Kerr accretion cases. The results demonstrate the designed high-order accuracy in smooth regimes and robust performance for demanding relativistic flows on curved stationary backgrounds.

==> sections/03b_face_ec.tex <==
\section{Entropy-stable DG spectral element discretization}
\label{sec:dgsem}

The continuous entropy conditions in Sections~\ref{sec:wform}--\ref{sec:entropy}
are inherited from the relativistic fluid equations.  We now introduce the
additional algebra needed to reproduce that structure discretely.  This is
the first point at which entropy variables, entropy potentials, and an
entropy-adapted parametrization of the stationary geometry are required.

\subsection{Entropy variables and stationary geometry identities}
\label{sec:entropy-algebra}

Let $d$ denote the number of active spatial coordinates.  For the reduced
models of Section~\ref{sec:entropy}, $d=2$.  Recall
$W=j\uhat$ and define
\begin{equation}
 \sigma:=\frac1d\log j,
 \qquad
 A_{ai}:=\alpha j\Theta_{ai},
 \qquad
 C^i:=j\beta^i,
 \qquad
 Y:=(\sigma,A,C).
 \label{eq:Y}
\end{equation}
This is an invertible parametrization of the stationary active geometry:
\begin{equation}
 \begin{aligned}
 j&=e^{d\sigma},&
 \alpha&=\left(\frac{\det A}{j^{d-1}}\right)^{1/d},&
 \Theta&=\frac{A}{\alpha j},\\
 \gamma&=(\Theta^T\Theta)^{-1},&
 \beta^i&=\frac{C^i}{j}.&&
 \end{aligned}
 \label{eq:Y-inverse}
\end{equation}
Only the upper-triangular entries of $A$ are independent.

The W-form entropy density can be viewed as
\begin{equation}
 \eta(W,Y)=j\widehat\eta(W/j).
 \label{eq:entropy}
\end{equation}
Holding the geometry fixed gives the same entropy variables as for the local
SRHD state.  With $\zeta=\rho/p$ and $K_a=L\vhat_a$,
\begin{equation}
 V:=\nabla_W\eta=
 \begin{pmatrix}
 \dfrac{\Gamma-s}{\Gamma-1}+\zeta\\
 \zeta K_a\\
 -\zeta L
 \end{pmatrix}.
 \label{eq:entropy-variables}
\end{equation}
Define the local temporal and directional entropy potentials by
\begin{equation}
 \Phi=V^T\uhat-\widehat\eta,
 \qquad
 \psi_a=V^T\fhat^a-\widehat q^a,
 \qquad
 \widehat q^a=\vhat_a\widehat\eta.
 \label{eq:local-potentials-definition}
\end{equation}
A direct calculation gives
\begin{equation}
 \Phi=D,
 \qquad
 \psi_a=D\vhat_a.
 \label{eq:potentials}
\end{equation}
The coordinate entropy potential is therefore
\begin{equation}
 \Psi^i:=V^TH^i-q_\eta^i=A_{ai}\psi_a-C^i\Phi.
 \label{eq:coordinate-entropy}
\end{equation}

The explicit source \eqref{eq:w-source-explicit} is linear in first spatial
derivatives of the stationary geometry.  Rewriting the same source in the
coordinates $Y=(\sigma,A,C)$ gives
\begin{equation}
 \mathcal S_W=
 B_\sigma^i\partial_i\sigma
 +B_{A_{ak}}^i\partial_iA_{ak}
 +B_{C^k}^i\partial_iC^k.
 \label{eq:Y-source}
\end{equation}
The following contractions are the only parts of the coefficient vectors
needed by the entropy analysis.
\begin{lemma}[Active-geometry source contractions]
\label{lem:source-contractions}
At fixed $W$,
\begin{equation}
 V^TB_\sigma^i=0,
 \qquad
 V^TB_{A_{ak}}^i=\delta_{ik}\psi_a,
 \qquad
 V^TB_{C^k}^i=-\delta_{ik}\Phi.
 \label{eq:source-contractions}
\end{equation}
\end{lemma}
\begin{proof}
For any stationary geometry coordinate $y$, continuous entropy compatibility
implies
\begin{equation}
 V^TB_y^i
 =V^T\left.\frac{\partial H^i}{\partial y}\right|_W
 -\left.\frac{\partial q_\eta^i}{\partial y}\right|_W.
 \label{eq:fixed-W-intrinsic}
\end{equation}
At fixed $W,A,C$, a variation of $\sigma$ changes only the local state
$\uhat=W/j$, and state compatibility cancels the corresponding physical- and
entropy-flux derivatives.  At fixed $W,\sigma$, the coefficients $A$ and $C$
enter $H^i$ and $q_\eta^i$ linearly, giving the remaining identities.
\end{proof}

\subsection{Unified notation for the physical reduction measure}
\label{sec:weighted-physical-coefficients}

For the numerical formulation it is convenient to use a single symbol for
the physical measure appearing in the conservative state.  We set
\begin{equation}
 \varpi=
 \begin{cases}
  1,&\text{for an unreduced/intrinsic W-form},\\
  w,&\text{for the symmetry-reduced models of Section~\ref{sec:entropy}},
 \end{cases}.
 \label{eq:physical-weight}
\end{equation}
Thus $\varpi$ is not an arbitrary numerical weight in the present paper; it
is either unity or the physically derived suppressed-direction factor.  It
may have a simple zero on a symmetry-axis boundary and is positive in the
interior.
Define
\begin{equation}
 \mathbb W:=\varpi W,
 \qquad
 \mathbb H^i:=\varpi H^i,
 \label{eq:weighted-state-flux}
\end{equation}
Both the general W-form of Section~\ref{sec:wform} and the reduced form of
Section~\ref{sec:entropy} can then be written as
\begin{equation}
 \partial_t\mathbb W+\partial_i\mathbb H^i
 =\varpi\mathcal S_W+P_\perp^i\partial_i\varpi.
 \label{eq:balance-law}
\end{equation}
For the reduced models the index $i$ in this section runs over the two active
coordinates.

The corresponding entropy pair is
\begin{equation}
 \mathbb\eta(\mathbb W,Y,\varpi)
 =\varpi\eta(\mathbb W/\varpi,Y),
 \qquad
 \mathbb q_\eta^i=\varpi q_\eta^i,
 \label{eq:weighted-entropy-pair}
\end{equation}
and entropy-admissible weak solutions satisfy
\begin{equation}
 \partial_t\mathbb\eta+\partial_i\mathbb q_\eta^i\le0,
 \label{eq:continuous-weighted-entropy}
\end{equation}
with equality for smooth solutions.  At fixed $Y$ and $\varpi$,
\begin{equation}
 \nabla_{\mathbb W}\mathbb\eta=V,
 \label{eq:weighted-entropy-variables}
\end{equation}
and
\begin{equation}
 \frac{\partial\mathbb q_\eta^i}{\partial\mathbb W}
 =V^T\frac{\partial\mathbb H^i}{\partial\mathbb W}.
 \label{eq:weighted-state-compatibility}
\end{equation}
The weighted entropy potential and temporal Legendre density are
\begin{equation}
 \mathbb\Psi^i
 =V^T\mathbb H^i-\mathbb q_\eta^i
 =\varpi\Psi^i,
 \label{eq:weighted-coordinate-potential}
\end{equation}
\begin{equation}
 V^T\mathbb W-\mathbb\eta=\varpi j\Phi.
 \label{eq:weighted-temporal-legendre-density}
\end{equation}

Direct substitution of \eqref{eq:suppressed-w-source} gives the key
continuous contraction
\begin{equation}
 V^TP_\perp^i=\Psi^i.
 \label{eq:weight-source-contraction}
\end{equation}
A componentwise verification is recorded in
Appendix~\ref{app:symmetry-reduction}.

For later flux differencing, absorb the physical measure into the coefficients
multiplying the local SRHD building blocks:
\begin{equation}
 A^\varpi_{ai}:=\varpi A_{ai},
 \qquad
 C_\varpi^i:=\varpi C^i.
 \label{eq:weighted-coordinate-coefficients}
\end{equation}
Then
\begin{equation}
 \mathbb H^i=A^\varpi_{ai}\fhat^a-C_\varpi^i\uhat,
 \qquad
 \mathbb\Psi^i=A^\varpi_{ai}\psi_a-C_\varpi^i\Phi.
 \label{eq:weighted-coordinate-physical-flux}
\end{equation}
The finite intrinsic coefficients $A$ and $C$ are retained separately; they
are never reconstructed by dividing $A^\varpi$ or $C_\varpi$ by $\varpi$.

Multiplying \eqref{eq:Y-source} by $\varpi$ and including the physical
suppressed source gives, before reparametrization,
\begin{equation}
 \mathbb S=
 \varpi B_\sigma^i\partial_i\sigma
 +\varpi B_{A_{ak}}^i\partial_iA_{ak}
 +\varpi B_{C^k}^i\partial_iC^k
 +P_\perp^i\partial_i\varpi.
 \label{eq:weighted-source-original-coordinates}
\end{equation}
Using the product rule in the forward direction, the same physical source is
\begin{equation}
 \mathbb S=
 \varpi B_\sigma^i\partial_i\sigma
 +B_{A_{ak}}^i\partial_iA^\varpi_{ak}
 +B_{C^k}^i\partial_iC_\varpi^k
 +R_\varpi^i\partial_i\varpi,
 \label{eq:weighted-source-reparameterization}
\end{equation}
where
\begin{equation}
 R_\varpi^i
 =P_\perp^i
 -B_{A_{ak}}^iA_{ak}
 -B_{C^k}^iC^k.
 \label{eq:weighted-weight-residual}
\end{equation}
For $\varpi=1$ the weight-derivative term vanishes.  For $\varpi=w$,
Eqs.~\eqref{eq:source-contractions} and \eqref{eq:weight-source-contraction}
give
\begin{equation}
 V^TR_\varpi^i
 =\Psi^i-A_{ai}\psi_a+C^i\Phi=0.
 \label{eq:weighted-weight-residual-contraction}
\end{equation}
The weighted active source contractions are correspondingly
\begin{equation}
 V^T(\varpi B_\sigma^i)=0,
 \qquad
 V^TB_{A_{ak}}^i=\delta_{ik}\psi_a,
 \qquad
 V^TB_{C^k}^i=-\delta_{ik}\Phi.
 \label{eq:weighted-source-contractions}
\end{equation}

\subsection{Local SRHD entropy-conservative building blocks}
\label{sec:local-ec-building-blocks}

For two admissible endpoints, recover the local states from
\begin{equation}
 \widehat U_L=\frac{\mathbb W_L}{\varpi_Lj_L},
 \qquad
 \widehat U_R=\frac{\mathbb W_R}{\varpi_Rj_R}.
 \label{eq:weighted-local-state-recovery}
\end{equation}
Let $\uhat_{LR}^{\#}$ be a symmetric, consistent temporal state and let
$\fhat_{LR}^{a,\EC}$ be a symmetric, consistent directional flux satisfying
\begin{equation}
 \jump V^T\uhat_{LR}^{\#}=\jump\Phi,
 \qquad
 \jump V^T\fhat_{LR}^{a,\EC}=\jump{\psi_a}.
 \label{eq:local-tadmor}
\end{equation}
Closed dimension-independent formulas based on arithmetic and logarithmic
means are collected in Appendix~\ref{app:local-ec} and agree with the SRHD
entropy-conservative constructions in
Refs.~\cite{BhoriyaKumar2020,DuanTang2019,BiswasKumar2022}.

\subsection{Conforming-face entropy-conservative flux}
\label{sec:physical-face-ec}

On a conforming physical face the prescribed spacetime geometry, the physical
reduction measure, and the physical normal are single-valued.  Hence the
shared-geometry specialization
\begin{equation}
 H_{LR}^{i,\#}
 :=A_{ai,f}\fhat_{LR}^{a,\EC}-C_f^i\uhat_{LR}^{\#},
 \qquad
 \mathbb H_{LR}^{i,\#}:=\varpi_fH_{LR}^{i,\#}
 \label{eq:shared-geometry-coordinate-ec}
\end{equation}
satisfies
\begin{equation}
 \jump V^T\mathbb H_{LR}^{i,\#}
 =\varpi_f\left(A_{ai,f}\jump{\psi_a}-C_f^i\jump\Phi\right)
 =\jump{\mathbb\Psi^i}.
 \label{eq:shared-geometry-coordinate-tadmor}
\end{equation}
This face specialization should not be confused with the mapped volume flux
introduced below, where spacetime, physical-reduction, and computational
geometry vary between volume nodes.

